High-Speed Dynamic 3D Imaging with Sensor Fusion Splatting

Capturing and reconstructing high-speed dynamic 3D scenes has numerous applications in computer graphics, vision, and interdisciplinary fields such as robotics, aerodynamics, and evolutionary biology. However, achieving this using a single imaging modality remains challenging. For instance, traditional RGB cameras suffer from low frame rates, limited exposure times, and narrow baselines. To address this, we propose a novel sensor fusion approach using Gaussian splatting, which combines RGB, depth, and event cameras to capture and reconstruct deforming scenes at high speeds. The key insight of our method lies in leveraging the complementary strengths of these imaging modalities: RGB cameras capture detailed color information, event cameras record rapid scene changes with microsecond resolution, and depth cameras provide 3D scene geometry. To unify the underlying scene representation across these modalities, we represent the scene using deformable 3D Gaussians. To handle rapid scene movements, we jointly optimize the 3D Gaussian parameters and their temporal deformation fields by integrating data from all three sensor modalities. This fusion enables efficient, high-quality imaging of fast and complex scenes, even under challenging conditions such as low light, narrow baselines, or rapid motion. Experiments on synthetic and real datasets captured with our prototype sensor fusion setup demonstrate that our method significantly outperforms state-of-the-art techniques, achieving noticeable improvements in both rendering fidelity and structural accuracy.

==> conf/packages.tex <==
\RequirePackage[english]{babel}                  %
\RequirePackage{xspace}                          %
\RequirePackage{xpunctuate}                      %

\RequirePackage{ifthen}                          %
\RequirePackage{soul}                            %
\RequirePackage{xargs}                           %

\RequirePackage{color}                           %

\RequirePackage{amsmath}                         %
\RequirePackage{bm}                              %

\RequirePackage[toc,page,titletoc]{appendix}     %
\RequirePackage[capitalize,nameinlink]{cleveref} %
\crefname{supp}{Supplement}{Supplements}     %



\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{bm}
\RequirePackage{graphicx}
\RequirePackage{xcolor}
\RequirePackage{soul}
\RequirePackage{float}
\RequirePackage{makecell}

\RequirePackage[export]{adjustbox}

\RequirePackage{caption}                         %
\RequirePackage{subcaption}                          %

\RequirePackage{arydshln}

